Exploring Recurrent, Memory and Attention Based Architectures for Scoring Interactional Aspects of Human-Machine Text Dialog

An important step towards enabling English language learners to improve their conversational speaking proficiency involves automated scoring of multiple aspects of interactional competence and subsequent targeted feedback. This paper builds on previous work in this direction to investigate multiple neural architectures -- recurrent, attention and memory based -- along with feature-engineered models for the automated scoring of interactional and topic development aspects of text dialog data. We conducted experiments on a conversational database of text dialogs from human learners interacting with a cloud-based dialog system, which were triple-scored along multiple dimensions of conversational proficiency. We find that fusion of multiple architectures performs competently on our automated scoring task relative to expert inter-rater agreements, with (i) hand-engineered features passed to a support vector learner and (ii) transformer-based architectures contributing most prominently to the fusion.

==> lstm.tex <==
\begin{table*}[tbh]
\caption{\label{tab:stats} {\it Human and machine score statistics - LSTM}}

\begin{tabular}{  l | c | c c | }
\hline
\multirow{2}{*}{Construct}	& \multirow{2}{*}{Sub-construct} &  \multicolumn{2}{|c|}{$LSTM_{attn}$}  \\
	&   & Accuracy & QW$\kappa$     \\
\hline
\multirow{4}{*}{Topic Development} &  Topic	&  70.0 & 0  \\
\cline{2-2}
& Elaboration	&      66.4 & 0 \\
\cline{2-2}
& Structure 	&    0 & 0 \\
\cline{2-2}
& Task	&    68.1 & 0 \\
\hline
\multirow{4}{*}{Interaction} &  Engagement	&   66.7 & 0 \\
\cline{2-2}
& Turn Taking	&   66.3 & 0 \\
\cline{2-2}
& Repair &   64.0 & 0  \\
\cline{2-2}
& Appropriateness  &  65.2 & 0 \\
\hline
\multicolumn{2}{c|}{Overall Holistic Performance}  &   67.0 & 0 \\
\hline
\end{tabular}
}

%\vspace{-1mm} [in some *CL conferences \vspace  = desk reject]
% \end{table*}
\end{table*}

From the POV of the SVM features (Section X) we notice lexicon features such as features depicting \emph{politeness} assists the classifier (e.g., especially for ``structure'' and ``turntaking'' constructs) to achieve better accuracy. 

The $BiLSTM_{attn}$ perform better compared to the vanilla stack BiLSTM networks for all the constructs. Attention was positioned on top of the stack networks, which means the attention mechanism is able to identify the key characteristics of the constructs. Further, we analyze the heat maps of the attention weights to interpret the models' performance. For brevity, we discuss only a couple of constructs here. 

Figure \ref{figure:task_attn} shows that the words representing particular actions, such as reviewing the slides or discussion have received the highest weights. Likewise, in Figure \ref{figure:appro_attn}, we observe  words representing positive and respectful tone (e.g., ``if you would look''; ``great yeah'') receiving higher attention weights.      


\begin{figure}[t]
\centering
\begin{framed}
\includegraphics[width=7cm]{task.pdf}
\caption{Attention weights depicting the \emph{task} construct}
\label{figure:task_attn}
\end{framed}
\end{figure}

\begin{figure}[t]
\centering
\begin{framed}
\includegraphics[width=7cm]{appro.pdf}
\caption{Attention weights depicting the \emph{Appropriateness} construct}
\label{figure:appro_attn}
\end{framed}
\end{figure}



